Neural Material: Learning Elastic Constitutive Material and Damping Models from Sparse Data

The accuracy and fidelity of deformation simulations are highly dependent upon the underlying constitutive material model. Commonly used linear or nonlinear constitutive material models only cover a tiny part of possible material behavior. In this work we propose a unified framework for modeling deformable material. The key idea is to use a neural network to correct a nominal model of the elastic and damping properties of the object. The neural network encapsulates a complex function that is hard to explicitly model. It injects force corrections that help the forward simulation to more accurately predict the true behavior of a given soft object, which includes non-linear elastic forces and damping. Attempting to satisfy the requirement from real material interference and animation design scenarios, we learn material models from examples of dynamic behavior of a deformable object's surface. The challenge is that such data is sparse as it is consistently given only on part of the surface. Sparse reduced space-time optimization is employed to gradually generate increasingly accurate training data, which further refines and enhances the neural network. We evaluate our choice of network architecture and show evidence that the modest amount of training data we use is suitable for the problem tackled. Our method is demonstrated with a set of synthetic examples.

==> algorithm-old.tex <==
\section{Method}
\label{sec:alg}

%\textcolor{red}{We need a short introduction here, but likewise, perhaps there needs to be a section on the acquisition and preparation of data.}

In the following subsections, we provide in depth details on the different steps of our algorithm.  Many of the steps involve approximations, and the captured surface trajectories may include noise.  As such, the general philosophy of the algorithm is to gradually learn the corrections necessary to produce forward simulations that replicate the capture trajectory. 

\subsection{Nominal Material Model and Assumptions}

Our deformable models are made of tetrahedra with linear shape functions, and the nominal material is a linear elastic model formulated using principal stretches \cite{Xu2015}.  The ensuing computation of the element stresses and vertex forces is straightforward.  The deformation gradient $F$ for each tetrahedron is then diagonalized by SVD, $F = U\hat{F}V^T$, and the Piola-Kirchoff stress is first computed with the principal stretches, $\hat{P}(\hat{F})=2\mu(\hat{F}-I)+\lambda tr(\hat{F}-I)I$, where $\mu$ and $\lambda$ are Lam� parameters.  The diagonal stress is then transformed back to the world frame, $P=U\hat{P}(\hat{F})V^T$.  An element's contribution to its vertex forces is $P B_m$, where $B_m$ is the inverse material space shape matrix (see \citet{Sifakis2012}).  Summing the contribution of all elements, we can build a large sparse matrix $\mathsf{B}$ that combines the entries in $U$, $V$, and $B_m$ which can be multiplied by the block vector of all element diagonal stresses $\mathsf{\hat{p}}$ to give a block vector of all vertex forces $\mathsf{f}$, that is,  $\mathsf{B\hat{p}=f}$.

For implicit integration, we note that the gradient of stress $P$ with respect to the deformation gradient $F$ can be computed by the product rule and a careful evaluation of the different terms \cite{Xu2015}.  In creating our synthetic test examples, we likewise use the stiffness in the computation of Raleigh damping, $(\alpha \mathsf{M} + \beta \mathsf{K})\mathsf{v}$.
%, with $\alpha = 0.01$ and $\beta=0.02$. % PGK <- Best to give the numbers in the results!!!
%
%\begin{equation}
%\frac{\partial P}{\partial F} = 
%\frac{\partial U}{\partial F} P(\hat{F}) V^T +
%U \frac{\partial{P(\hat{F})}}{\partial F} V^T +
%U P(\hat{F}) \frac{\partial{V^T}}{\partial F}.
%\end{equation}

%We further approximate the damping stress with the omission of the time derivatives of $U$ and $V$ assuming they are small. Thus, our nominal damping stress is computed as $U(2\beta\hat{\dot{F}}+\alpha tr(\hat{\dot{F}})I) V^T$.
% PGK: Irving comments about how this does not preserve angular momentum in Section 6.2
% PGK: Turns out we're not using this kind of damping at all, but the issue comes up 
% in another way as described below. 

Following \citet{Irving2004}, we transform the deformation gradient velocity $\dot{F}$ by the same $U$ and $V$ as $F$.  While the rotated velocity gradient is not generally diagonal, we set \smash{$\hat{\dot{F}}$} with only the diagonal terms of $U\dot{F}V^T$. 
%
The neural network computes correction to the Piola stress using the same rotations $U$ and $V$ as the nominal model, and corrects the elasticity and damping simultaneously. 
%In particular, note that we only provide principal stretches and the diagonal terms the diagonalized deformation gradient velocity \hat{\dot{F}}. 
Thus we define the function $N$ to be our neural network correction of the diagonal stress, \smash{$\Delta \hat{P} = N(\hat{F},\hat{\dot{F}})$}.
Using principal stretches and the diagonal deformation gradient velocity reduces the complexity of our function approximation problem.  As we will discussed later, 
the 6-input 3-output function approximation problem allows us to select a network architecture with a moderate number of hidden nodes, which can be trained with reasonable quantities of training data that we can easily produce.  

%  We describe how the nerual network augments this material model, and how we compute the stiffness matrix needed in implicit integration. 

We do not currently include Raleigh damping in our nominal model, thus the corrected stresses in the world frame are %computed as
\begin{equation}
P_n = U(\hat{P}(\hat{F}) + N(\hat{F},\hat{\dot{F}}))V^T,
\label{eq:force}
\end{equation}
and the gradient for implicit integration here includes a gradient of $N$, which is easily computed from the neural network function with automatic differentiation.


\subsection{Constrained Forward Simulation}

We use semi-implicit backward Euler integration for simulation.  While this choice of integrator has the disadvantage of time step dependent numerical damping, it is convenient due to the ease of implementation and stability.  At each step we solve the equation 
\begin{equation}
\mathsf{A} \Delta \mathsf{v} = h \mathsf{f}
\end{equation}
where $\mathsf{f} = \mathsf{B p_n} + \mathsf{f}_\text{ext}$, with $\mathsf{p_n}$ being the block vector of neural material stresses at the current time step, $\mathsf{f}_\text{ext}$ being the external gravity force, and $\mathsf{A = M - hD -h^2K}$ where $\mathsf{D}$ and $\mathsf{K}$ are assembled using the gradient of Equation \ref{eq:force}.  Many of our models are rigidly attached to the world, and we typically remove these degrees of freedom from the system.  Forward simulation is an important step in our fitting process as we use it to evaluate the performance of the current neural material estimate, which we do by monitoring the maximum vertex error compared to the ground truth trajectory observation.

The space-time constraints optimization needs a reasonable starting trajectory.  While the forward simulation with the current neural material estimate could serve this purpose, it is more valuable to simulate a trajectory constrained to follow the measurements.  We can divide the vertices into two groups, 
\begin{equation}
\begin{pmatrix}
\mathsf{A_{uu}} & \mathsf{A_{uc}} \\ \mathsf{A_{cu}} & \mathsf{A_{cc}}
\end{pmatrix}
\begin{pmatrix}
\Delta \mathsf{v_u} \\ \Delta \mathsf{v_c}
\end{pmatrix}
=
h
\begin{pmatrix}
\mathsf{f_u} \\ \mathsf{f_c}
\end{pmatrix}
\end{equation}
where we use subscript $u$ for unconstrained and $c$ for constrained.  The second block row can be discarded leaving us a smaller system to solve, namely,
\begin{equation}
\mathsf{A_{uu}} \Delta \mathsf{v_u} =  h\mathsf{f_u} - \mathsf{A_{uc}} \Delta \mathsf{v_c}.
\end{equation}
Here, $\Delta \mathsf{v_c}$ at time step $i$ is computed by a second order central finite difference, $h^{-1}(x_{i-1} - 2x_i + x_{i+1})$.  We solve these large sparse systems using PARDISO~\cite{pardiso-6.0a,pardiso-6.0b}.


\subsection{Space-Time Constraints Optimization}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bsfs}{\bm{\mathsf{s}}}
\newcommand{\bsfC}{\bm{\mathsf{C}}}
\newcommand{\bsfCf}{\bm{\mathsf{C_f}}}
\newcommand{\bsfCx}{\bm{\mathsf{C_x}}}

The partially scanned surface trajectory provides a rich source of information about the dynamics of the object.  The purpose of using a space-time optimization is to compute a set of gentle control forces that will correct our currently estimated neural material such that the simulation follows captured data.  While it makes sense to inject a control stress at each element, the naive approach of providing a control force at each vertex is extremely easy and permits an easier solution.  
However, as described below, this not precisely what we do, as we do not explicitly include control forces in our optimization.
% i.e., think non-conservitive type effects??

The original space-time constraints approach \cite{Witkin1988} applied to our problem involves minimizing control forces $R = \norm{\bm{\mathsf{f}}}$, where $\bm{\mathsf{f}}$ is a block vector assembling all control forces on vertices $\mathbf{f}_i$ for each time step $i$.  The variables over which we are optimizing are these forces $\bm{\mathsf{f}}$ along with the position  $\bm{\mathsf{x}}$ of all 
%unobserved vertices across all time steps $\bm{\mathsf{x}}_u$.  These variables can be assembled into 
vertices across all time steps.  These variables are assembled into 
a vector,
\begin{equation}
\bsfs = \begin{pmatrix} \bm{\mathsf{f}} \\ \bm{\mathsf{x}} \end{pmatrix}.
%S = \begin{pmatrix} \bm{\mathsf{f}} \\ \bm{\mathsf{x}}_u \end{pmatrix}.
\end{equation}
The constraints include a vector valued constraint function for each time step $i$,
\begin{equation}
\mathsf{C}_i \equiv 
h^{-2}\mathsf{M}(\mathsf{x}_{i-1} - 2\mathsf{x}_i + \mathsf{x}_{i+1} ) 
- \mathsf{B}_{i+1} \mathsf{p}_{\mathsf{n},i+1} 
- \mathsf{f}_{ext} -\mathsf{f}_{i+1}.
%%%\hat{P}(\hat{F_j}) + N(\hat{\dot{F_j}},\hat{\dot{F_j}}) ) 
\label{eq:physicsconstraint}
\end{equation}
Notice that we make these constraints correspond to our %semi-implicit backward Euler 
forward integration method by evaluating the force term at the
end of the time step.  
%That is, we compute $\mathsf{B}_i \mathsf{p}_{\mathsf{n}i}$  using $\mathsf{B}_i$ using the $U$ and $V$ from the SVDs of the deformation gradient at time step $i$, but otherwise computing the stress by Equation~\ref{eq:force} with the deformation gradient at the next time step and $h^{-1}(\mathsf{x}_{i+1} - \mathsf{x}_i)$ for the deformation gradient velocity.
We write these force constraints as a block vector $\bsfCf$.
%\pk{HUH? INDEXING DETAILS CORRECT? NECESSARY?}
% PGK I'M NOT EXACTLY SURE ABOUT THE INDEXING... UNNECESSARY DETAILS?}.  
%%% PGK :  Huh?  Subtle difference about indexing here... not sure exactly what is done!

We also have position constraints $\bsfCx$ that come from capture data, as well as boundary constraints (e.g., constraints for the start and end pose based on the scenario, for instance, a static equilibrium pose computed from available information).  These constraints trivially state that some components of the vector $\bm{\mathsf{x}}$ must take on a specific value.  

In the traditional approach, we would solve for $\hat{\bsfs}$ in
\begin{equation}
\frac{\partial^2 R}{\partial \bsfs^2} \hat{\bsfs} = -\frac{\partial R}{\partial \bsfs} 
\end{equation}
and then subsequently compute a projection onto the constraints by solving for $\tilde{\bsfs}$ in 
\begin{equation}
-\bsfC = \frac{\partial \bsfC}{\partial \bsfs}  (\tilde{\bsfs} + \hat{\bsfs}),
\label{eq:ST2}
\end{equation}
where $\bsfC$ contains both physics constraints $\bsfCf$ and position constraints $\bsfCx$.
In our formulation, by choosing vertex control forces instead of stresses, $\hat{\bsfs}$ will always be zero.  Furthermore, we simplify the solution of Equation~\ref{eq:ST2} to 
\begin{equation}
\frac{\partial \bsfCf}{\partial \bm{\mathsf{x}}} \Delta {\bm{\mathsf{x}}} = -\bsfCf, 
\label{eq:ourSTC}
\end{equation}
which allows us to focus on changing only the positions while minimizing the violation of physics constraints.
We iterate on solving Equation~\ref{eq:ourSTC}, updating our solution $\bm{\mathsf{x}}^* \leftarrow \bm{\mathsf{x}}^* + \zeta_\mathsf{x} \Delta \bm{\mathsf{x}}$, using a step damped by factor $\zeta_\mathsf{x}$, typically in the range 0.1 to 0.5, 
and then directly setting all constrained positions $\bm{\mathsf{x}}_\mathsf{c}$ in $\bm{\mathsf{x}}^*$ to satisfy
$\bsfCx$.

The computation of the gradient of $\bsfCf$ in Equation~\ref{eq:ourSTC} has a very simple part that links vertices at different times steps through the acceleration term, and a more complex part where the chain rule must be applied to compute the force gradient, which includes a contribution from the neural network.  This second part sprinkles off diagonal terms into the matrix linking vertices that are adjacent to a common element.  While the constraint gradient matrix is very large, it is also very sparse, and we compute the solution using the Eigen library's sparse conjugate gradient implementation.

Once our solution $\bm{\mathsf{x}}^*$ has converged, which we check by monitoring the physics constraints, it is likewise the physics constraints in Equation~\ref{eq:physicsconstraint} from which we compute the necessary control forces to correct our current neural material model.

%\begin{pmatrix}
%\frac{\partial \mathsf{C_f}{\partial \bm{\mathsf{f}} & \frac{\partial \mathsf{C_f}{\partial \bm{\mathsf{x}} \\	
%\frac{\partial \mathsf{C_x}{\partial \bm{\mathsf{f}} & \frac{\partial \mathsf{C_x}{\partial \bm{\mathsf{x}} \\
%\end{pmatrix}

%\begin{equation}
%C = \begin{pmatrix} C_p \\ C_x \end{pmatrix}
%\end{equation}

%physics constraints and position constraints... 
%partial C partial s = 

These are big space-time constraints optimization problems.  While we are currently assuming homogeneous material in our simulated objects, given that we are working with unknown non-linear constitutive models it is not straightforward to apply recent material parameter estimation techniques \cite{Chen2017}, or to find solutions with model reduction \cite{Schulz2014}.  In cases where the problem is too large and ill-conditioned to efficiently solve, we note that the constrained forward simulation can prove to be a sufficient source of information to produce training data that can improve the neural material model. The idea here is that with a long enough trajectory, the start and end of the space-time constraints become less important as the partial surface scan trajectory can be dense enough to be the primary source of information about the object dynamics.  In contrast to the space-time optimization solution, here, the control forces that we can identify for training are exclusively the constraint forces necessary to have the observed trajectory followed in the forward simulation.  The disadvantage of this approach is that our algorithm converges much more slowly.  We discuss this further in Section \ref{sec:results}. 


\subsection{Training Data Preparation}

%%% PGK: THIS MAY SEEM EARLY IN THE .tex BUT IT MAKES IT APPEAR ON PAGE 5


The result of our space-time constraints optimization (and likewise the constrained forward simulation in some cases), provides vertex control forces to correct our model, but we need stresses to train our neural network.
 
% Easy fix
At every time step $i$, we must identify stresses that produce the desired control forces $\mathsf{f}_i$.  While the linear system $\mathsf{B\hat{p}=f}$ has a tall matrix for a single tetrahedron, typical larger systems will have more tetrahedra than vertices and $\mathsf{B}$ will be a fat matrix.  Indeed it is possible for different combinations of stresses to produce the same force.  However, $\mathsf{B}$ also has deficient row rank as there can be forces that cannot be realized by internal stresses alone.
 (For instance, a constant force on all vertices as would be produced by gravity cannot be produced by internal stresses.)  
 Thus, we compute the stresses as a least squares problem using LSQR \cite{Paige1982}, which finds $\mathsf{\hat{p}^*}$ that minimizes  $\norm{\mathsf{\hat{p}}}$ subject to 
$\mathsf{B^TB \hat{p} = B^Tf}$ using an iterative algorithm that exploits sparsity and avoids assembling the product $\mathsf{B^TB}$.

During the training process, the neural network will have developed an estimate for the required correction to the diagonal Piola stress $\Delta \mathsf{\hat{P}}$.  Thus we combine the current network output with our newly estimated stress corrections.  For each time step, we solve the least squares problem, and then for each element extract its stress $\hat{P}^*$ from the block vector $\mathsf{\hat{p}}^*$, from which we then assemble a training data pair
\begin{equation}
\left(\hat{F}, \hat{\dot{F}}\right), \ \
\left(N(\hat{F},\hat{\dot{F}})+\zeta_P\hat{P}^* \right),
\end{equation}
where the factor $\zeta_P$, typically set to $0.1$, allows us to take smaller conservative steps towards learning the correction.

%\pk{Could describe the alternative information loosing strategy of solving
%$\mathsf{B^TB\hat{p}=B^T(f + B N)}$ ?}



% SCRAPS:  (can probably be deleted...)
%For every time step, we have the solution to the least squares solve, 
%every element and every time step, we can now compute $\hat{F}$, %$\hat{\dot{F}}$, and $N(\hat{F},\hat{\dot{F}})+\hat{P}^*$%
%	At each time step
%\mathsf{\hat{p}}
%  This can be done by solving for a the minimum  satisfying , except that the control forces by the space time constraints system will not be compatible linear system.
%
%The space time constraints simulation will allow us to identify an update to these corrections  
%
%If $A$ has low column rank, the solution is not unique. LSQR returns the solution of minimum length. Thus for under-determined systems, it minimizes $x$ subject to $A^TAx=A^Tb$, which it does without forming the product $A^TA$ .



%Subtract the NN's current force contribution at vertices from the gentle control forces, and then project back to stresses by solving a least squares problem.  Thus, we want the Piola stress correction in each element $Ap=f$.  The matrix can be fat or skinny depending on the topology of the mesh, but regardless the shape, the image of the linear map $A$ is not expected to map to cover possible forces (for instance, there is no possible combination of stresses that can produce a constant force field).  By left multiplying by $A^T$, we ensure that we are finding the minimum norm $p$ which produces the realizable portion of $f$.  To solve the problem $A^TAp=A^Tf$ we assemble the large system matrix at each step, and use a sparse iterative method (or a direct method?) which can deal with the indefiniteness of $A^TA$.


% why not A = USV^T.. VSU^TUSV p = VSU^T f   ARGH... why is this not the same!? 


